Thermometry of ultracold atoms via non-equilibrium work distributions

Estimating the temperature of a cold quantum system is difficult. Usually, one measures a well-understood thermal state and uses that prior knowledge to infer its temperature. In contrast, we introduce a method of thermometry that assumes minimal knowledge of the state of a system and is potentially non-destructive. Our method uses a universal temperature-dependence of the quench dynamics of an initially thermal system coupled to a qubit probe that follows from the Tasaki-Crooks theorem for non-equilibrium work distributions. We provide examples for a cold-atom system, in which our thermometry protocol may retain accuracy and precision at subnanokelvin temperatures.

==> Explanation_of_mat_files <==
The two files

mixedCharFunc_L11_J1_U4_mu-1_temp1_impSite6_lambdaI0_lambdaF2_tQ0.1_uMax20_du0.04_dir1_nMax3_chi200.mat
mixedCharFunc_L11_J1_U4_mu-1_temp1_impSite6_lambdaI0_lambdaF2_tQ0.1_uMax20_du0.04_dir-1_nMax3_chi200.mat

contain the numerical data obtained by our calculation of the characteristic function for the forward and backward work distributions for the strongly-interacting Bose-Hubbard model, performed using tensor network methods (see main text and supplemental material for details).

The array charFunc stores the value of the characteristic function \chi(u) at 501 values of u between 0 and 20, corresponding to a timestep of 0.04. All times are in units of hbar/J with J the hopping energy in the Bose-Hubbard model. All other values are given in the main text and supplemental materials.

